TreeSketchNet: From Sketch To 3D Tree Parameters Generation

3D modeling of non-linear objects from stylized sketches is a challenge even for experts in Computer Graphics (CG). The extrapolation of objects parameters from a stylized sketch is a very complex and cumbersome task. In the present study, we propose a broker system that mediates between the modeler and the 3D modelling software and can transform a stylized sketch of a tree into a complete 3D model. The input sketches do not need to be accurate or detailed, and only need to represent a rudimentary outline of the tree that the modeler wishes to 3D-model. Our approach is based on a well-defined Deep Neural Network (DNN) architecture, we called TreeSketchNet (TSN), based on convolutions and able to generate Weber and Penn parameters that can be interpreted by the modelling software to generate a 3D model of a tree starting from a simple sketch. The training dataset consists of Synthetically-Generated \revision{(SG)} sketches that are associated with Weber-Penn parameters generated by a dedicated Blender modelling software add-on. The accuracy of the proposed method is demonstrated by testing the TSN with both synthetic and hand-made sketches. Finally, we provide a qualitative analysis of our results, by evaluating the coherence of the predicted parameters with several distinguishing features.

==> samples/imgs_low/handMade_with_tag_efficientnet/1_acer/acer_handMade_params.tex <==
\begin{tabular}{|l |l|} 
 \cline{2 -2}
 \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{OUTPUT}\\
 \hline
$GBS$ & $[3.5, -1.82]$\\[1pt]
$CBH$ & $0.29$ \\[1pt]
$N_{TF}$ & $1$\\[1pt]
$BD$ & $1.5$\\[1pt]
$N_B$ & $[0, 54]$\\[1pt]
$\phi_{FIB}$ & $[0.15, -12.4]$\\[1pt]
$\phi_{SIB}$ & $[0.33, -3.14]$\\[1pt]
% Down Angle & $[-0.88, 25.47]$\\[1pt]
% Leaf  Down Angle & $31.76$\\[1pt]
% Leaf Rotate Angle & $133.59$\\[1pt]
% Leaf Scale & $0.43$\\[1pt]
% Leaf Scale X & $0.79$\\[1pt]
% Leaf Scale T & $0.12$\\[1pt]
% Leaf Angle & $-12.23$\\[1pt]
% Leaves & $148$\\[1pt]
% Length & $[0.8, 0.6]$\\[1pt]
$N_L$ & $2$\\[1pt]
$B_{BW}$ & $0$\\[1pt]
% Rotate Angle& $[161.44, 136.3]$\\
% Scale & $4.98$\\
% Radius Scale & $1$\\
% Split Angle & $[17.72, 17.2]$\\
% % Split Bias & $0.55$\\
% Split Height & $0.48$\\
 \hline
 accuracy & $\approx 90\%$\\
 \hline
\end{tabular}

==> samples/imgs_low/handMade_with_tag_efficientnet/2_palm/palm_handMade_params.tex <==
\begin{tabular}{|l |l|} 
 \cline{2 -2}
 \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{OUTPUT}\\
 \hline
$GBS$ & $[8.51, -0.2]$\\[3.5pt]
$CBH$ & $0.0$ \\[3.5pt]
$N_{TF}$ & $0$\\[3.5pt]
$BD$& $9.921$\\[3.5pt]
$N_B$ & $[0, 25]$\\[3.5pt]
$\phi_{FIB}$ & $[23.83, 51.3]$\\[3.5pt]
$\phi_{SIB}$ & $[-22.87, 15.71]$\\[3.5pt]
% Down Angle & $[0.23, 44.99]$\\
% Leaf  Down Angle & $39.62$\\
% Leaf Rotate Angle & $92.17$\\
% Leaf Scale & $1.28$\\
% Leaf Scale X & $0.07$\\
% Leaf Scale T & $0.87$\\
% Leaf Angle & $-5.27$\\
% Leaves & $195$\\
% Length & $[0.61, 0.37]$\\
$N_L$ & $2$\\[3.5pt]
$N_{BW}$ & $2$\\[3.5pt]
% Rotate Angle& $[245.05, 67.51]$\\
% Scale & $13.84$\\
% Radius Scale & $1.0$\\
% Split Angle & $[7.39, 0.87]$\\
% Split Bias & $0.03$\\
% Split Height & $0.01$\\
\hline
 accuracy & $\approx 90\%$\\
 \hline
\end{tabular}

==> samples/imgs_low/handMade_with_tag_efficientnet/3_pine/pine_handMade_params.tex <==
\begin{tabular}{|l |l|} 
 \cline{2 -2}
 \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{OUTPUT}\\
 \hline
$GBS$ & $[2.0, 0.0, 0.45]$\\[3pt]
$CBH$ & $0.08$ \\[3pt]
$N_{TF}$ & $0$\\[3pt]
$BD$ & $1.619$\\[3pt]
$N_B$ & $[0, 36, 7]$\\[3pt]
$\phi_{FIB}$ & $[-9.37, -36.12, -28.9]$\\[3pt]
$\phi_{SIB}$ & $[10.9, -2.1, -1.31]$\\[3pt]
% Down Angle & $[85.0, 105.53, 44.05]$\\
% Leaf  Down Angle & $65.35$\\
% Leaf Rotate Angle & $133.04$\\
% Leaf Scale & $0.23$\\
% Leaf Scale X & $0.04$\\
% Leaf Scale T & $0.26$\\
% Leaf Angle & $-11.19$\\
% Leaves & $480$\\
% Length & $[0.99, 0.33, 0.73]$\\
$N_L$ & $3$\\[3pt]
$N_{BW}$ & $5$\\[3pt]
% Rotate Angle& $[197.28, 136.07, -80.48]$\\
% Scale & $4.08$\\
% Radius Scale & $1.0$\\
% Split Angle & $[0.24, 21.23, 23.84]$\\
% Split Bias & $0.04$\\
% Split Height & $0.22$\\
\hline
 accuracy & $\approx 94\%$\\
 \hline
\end{tabular}

==> samples/imgs_low/handMade_with_tag_efficientnet/4_cherry/cherry_handMade_params.tex <==
\begin{tabular}{|l |l|} 
 \cline{2 -2}
 \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{OUTPUT}\\
 \hline
$GBS$ & $[0.0, 0.06, 0.2, 0.02]$\\[4pt]
$CBH$ & $0.49$ \\[4pt]
$N_{TF}$ & $1$\\[4pt]
$BD$ & $1.965$\\[4pt]
$N_B$ & $[0, 39, 39, 10]$\\[4pt]
$\phi_{FIB}$ & $[18.1, -2.16, -1.4, -19.5]$\\[4pt]
$\phi_{SIB}$ & $[22.6, 11.7, 3.1, -0.04]$\\[4pt]
% Down Angle & $[1.25, 48.63, 47.39, 30.81]$\\
% Leaf  Down Angle & $-44.34$\\
% Leaf Rotate Angle & $271.7$\\
% Leaf Scale & $0.12$\\
% Leaf Scale X & $1.0$\\
% Leaf Scale T & $0.1$\\
% Leaf Angle & $17.56$\\
% Leaves & $1$\\
% Length & $[0.68, 0.6, 0.15, 0.47]$\\
$N_L$ & $4$\\[4pt]
$N_{BW}$ & $0$\\[4pt]
% Rotate Angle& $[146.73, 111.71, 104.46, 274.07]$\\
% Scale & $11.65$\\
% Radius Scale & $1.0$\\
% Split Angle & $[19.77, 33.98, 39.1, 55.23]$\\
% Split Bias & $0.97$\\
% Split Height & $0.54$\\
\hline
 accuracy & $\approx 90\%$\\
 \hline
\end{tabular}

==> samples/imgs_low/handMade_with_tag_efficientnet/5_bonsai/bonsai_handMade_params.tex <==
\begin{tabular}{|l |l|} 
 \cline{2 -2}
 \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{OUTPUT}\\
 \hline
$GBS$ & $[0, 1, 0, 0]$\\[5pt]
$CBH$ & $0.2$ \\[5pt]
$N_{TF}$ & $0$\\[5pt]
$BD$ & $1.4807$\\[5pt]
$N_B$ & $[0, 15, 15, 10]$\\[5pt]
$\phi_{FIB}$ & $[-62, 145, -1.4, -23]$\\[5pt]
$\phi_{SIB}$ & $[63, -136, -99, -0.6]$\\[5pt]
% Down Angle & $[1.92, 42.24, 2.29, 1.52]$\\
% Leaf  Down Angle & $49.07$\\
% Leaf Rotate Angle & $136.36$\\
% Leaf Scale & $0.06$\\
% Leaf Scale X & $0.49$\\
% Leaf Scale T & $0.11$\\
% Leaf Angle & $0.44$\\
% Leaves & $44$\\
% Length & $[1.02, 0.59, 0.41, 0.48]$\\
$N_L$ & $4$\\[5pt]
$N_{BW}$ & $0$\\[5pt]
% Rotate Angle& $[183.96, 120.21, 128.94, 133.73]$\\
% Scale & $1.25$\\
% Radius Scale & $1.0$\\
% Split Angle & $[1.48, 18.48, 47.11, 1.06]$\\
% Split Bias & $1.89$\\
% Split Height & $0.0$\\
\hline
 accuracy & $\approx 94\%$\\
 \hline
\end{tabular}

==> sections/acknowledgments.tex <==
\section{Acknowledgments}\label{sec:acknowledgments}
%The authors thank NVIDIA’s Academic Research Team for providing the Titan Xp card under the Hardware Donation Program. Furthermore, they wish to thank all controlled experiment participants in providing us the sketches.
The authors thank the NVIDIA’s Academic Research Team for providing the Titan Xp card under the Hardware Donation Program. Furthermore, they wish to thank all of the participants in the controlled experiment  for providing us with the sketches.
